Enriching a CP-Net by Asymmetric Merging

Conditional ceteris paribus preference networks (CP-nets) are commonly used to capture qualitative conditional preferences. In many use cases, when the preferential structure of an agent is incomplete, information from other preferential structures (e.g. that of other users) preferences can be used to fill in the gaps. Earlier works proposed methods to symmetrically merge multiple incomplete CP-nets by means of voting semantics. However, the merged CP-net can contain preference relations that do not fit to a given user's original preference profile. This paper proposes an asymmetric merging (or enriching) method to obtain and fill-in preference relations of a user's CP-net from another CP-net in a way that preserves the original preference relations.

==> test.tex <==
\usepackage{amsthm, amsmath}

\usepackage{listings}
\usepackage[toc,page]{appendix}
\usepackage[hyphens]{url}
\usepackage{subfig}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{tikz}
\usepackage{comment}
\usetikzlibrary{shapes, arrows}

\tikzstyle{feature} = [circle, text centered, draw=black]
\tikzstyle{table1} = [rectangle, minimum width=3cm, minimum height=0.6cm, draw]
\tikzstyle{table2} = [rectangle split, rectangle split parts=2, minimum height=1.5cm, minimum width=3cm, draw, text centered]
\tikzstyle{table3} = [rectangle split, rectangle split parts=3, minimum height=2.25cm, minimum width=3cm, draw, text centered]
\tikzstyle{table4} = [rectangle split, rectangle split parts=4, minimum height=2.25cm, minimum width=3cm, draw, text centered]
\tikzstyle{table5} = [rectangle split, rectangle split parts=5, minimum height=2.25cm, minimum width=3cm, draw, text centered]
\tikzstyle{table7} = [rectangle split, rectangle split parts=7, minimum height=2.25cm, minimum width=3cm, draw, text centered]
\tikzstyle{table9} = [rectangle split, rectangle split parts=9, minimum height=2.25cm, minimum width=3cm, draw, text centered]
\tikzstyle{arrow} = [thick,->,>=stealth]

\begin{document}
\begin{figure} [h]
\centering
\input{images/tikz/cp-example_unfolded}
\caption{Example CP-net.} \label{fig:example_cp}
\end{figure}
\end{document}
